Model-Based Epistemic Variance of Values for Risk-Aware Policy Optimization

We consider the problem of quantifying uncertainty over expected cumulative rewards in model-based reinforcement learning. In particular, we focus on characterizing the variance over values induced by a distribution over Markov decision processes (MDPs). Previous work upper bounds the posterior variance over values by solving a so-called uncertainty Bellman equation (UBE), but the over-approximation may result in inefficient exploration. We propose a new UBE whose solution converges to the true posterior variance over values and leads to lower regret in tabular exploration problems. We identify challenges to apply the UBE theory beyond tabular problems and propose a suitable approximation. Based on this approximation, we introduce a general-purpose policy optimization algorithm, Q-Uncertainty Soft Actor-Critic (QU-SAC), that can be applied for either risk-seeking or risk-averse policy optimization with minimal changes. Experiments in both online and offline RL demonstrate improved performance compared to other uncertainty estimation methods.

==> sections/biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/carlos_luis}}]{Carlos
E. Luis} is a PhD candidate at Bosch Corporate Research and the Intelligent Autonomous Systems group
at the Technical University of Darmstadt. Previously, he received a BSc in Electronics Engineering
from University Simon Bolivar and a MSc in Aerospace Studies from University of Toronto. Before
joining Bosch, he worked as a software development engineer at Amazon. His research is focused in
sample-efficient reinforcement learning and uncertainty quantification.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/alessandro_bottero}}]{Alessandro
G. Bottero} is a PhD candidate at Bosch Corporate Research and the Intelligent Autonomous Systems
group at the Technical University of Darmstadt. Previously, he received a BSc in Physics from
Università degli studi di Pavia and a MSc in Theoretical Physics from Ludwig-Maximilians-Universität
of Munich. Before joining Bosch, he worked as a software consultant at TNG - Technology Consulting.
His research is focused in safe exploration in Bayesian optimization and reinforcement learning.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/julia_vinogradska}}]{Julia
Vinogradska} is a group leader in black-box optimization methods at Bosch Corporate Research. She
received a BSc and MSc degree in mathematics from the University of Stuttgart, and a PhD from the
Technical University of Darmstadt. She has received the Stiftung Werner von Siemens Ring
Jungwissenschaftler (junior scientist) award for the research conducted during her PhD studies.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/felix_berkenkamp}}]{Felix
Berkenkamp} is a lead research scientist and activity lead at Bosch Corporate Research. Previously,
he completed a PhD at ETH Zurich, for which he received the ELLIS PhD award. During his PhD studies,
he held a AI fellowship from the Open Philanthropy Project, was an Associated Fellow at the Max
Planck ETH Center for Learning systems and a postgraduate affiliate at the Vector institute. He
served as the workflow co-chair for ICML 2018, publication chair for ICML 2024, and completed research internships at Microsoft
Research and Deepmind. He is interested in the fundamental problems behind data-efficient and safe
reinforcement learning with the goal of enabling learning on real-world systems.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/jan_peters}}]{Jan
Peters} is a full professor (W3) for Intelligent Autonomous Systems at the Computer Science
Department of the Technische Universität Darmstadt and at the same time a research department head
at the German Research Center for Artificial Intelligence (DFKI). He has received a number of
awards, including in particular the Dick Volz Best 2007 US Ph.D. Thesis Runner-Up Award, the
Robotics: Science \& Systems - Early Career Spotlight, the INNS Young Investigator Award, and the
IEEE Robotics \& Automation Society's Early Career Award as well as numerous best paper awards. He
has received a prestigious ERC Starting Grant and was promoted to a fellow by many well-known
research associations (IEEE, AAIA, ELLIS). His PhD students have received prestigious PhD awards
including twice the Georges Giralt Award for best European Robotics PhD Thesis (and, additionally,
two more have been runner-up for that award).
\end{IEEEbiography}


==> tables/d4rl_mujoco.tex <==
\begin{table}[t]
\addtolength{\tabcolsep}{-2pt}
\renewcommand\arraystretch{1.5}
\small
\centering
\caption{D4RL final normalized scores for model-based RL algorithms. The highest average scores are
highlighted in light blue. MOPO$\star$ corresponds to our own implementation of the algorithm by
\citet{yu_mopo_2020}, while QU-SAC utilizes the \texttt{upper-bound} variance estimate and $M=2$.
For MOPO$\star$ and QU-SAC, we report the mean and standard deviation over five random seeds. The
scores for the original MOPO results are as reported by \citet{bai_pessimistic_2022}. We take the
results for COMBO \citep{yu_combo_2021}, RAMBO \citep{rigter_rambo-rl_2022} and CBOP
\citep{jeong_conservative_2023} from their corresponding papers.}
\label{tab:d4rl_sota_comp}
% Somehow table caption overlaps with toprule if no vspace is used.
\vspace{1ex}
\begin{tabular}{
  c@{\hspace{3pt}}l@{\hspace{5.0pt}}r@{\hspace{-0pt}}lr@{\hspace{-0.0pt}}lr@{\hspace{-0.0pt}}lr@{\hspace{-0.0pt}}lr@{\hspace{-0.0pt}}lr@{\hspace{-0.0pt}}lr
  }

\toprule

\multicolumn{1}{l}{} & & \multicolumn{2}{c}{MOPO} & \multicolumn{2}{c}{MOPO$\star$} &
\multicolumn{2}{c}{COMBO} & \multicolumn{2}{c}{RAMBO} & \multicolumn{2}{c}{CBOP} &
\multicolumn{2}{c}{\textbf{QU-SAC}}  \\

\midrule
\multirow{3}{*}{\rotatebox[origin=c]{90}{Random}} 

& HalfCheetah & 35.9 & $\pm$2.9  & 25.9 & $\pm$1.4 & 38.8 & $\pm$3.7& \colorbox{mine}{40.0} &
$\pm$2.3 & 32.8 & $\pm$0.4 & 30.5 & $\pm$1.2 \\

& Hopper & 16.7 & $\pm$12.2  & \colorbox{mine}{32.6} & $\pm$0.2  & 17.9 & $\pm$1.4 & 21.6 & $\pm$8.0
& 31.4 & $\pm$0.0 & 19.3 & $\pm$7.6 \\

& Walker2D & 4.2 & $\pm$5.7  & 1.0 & $\pm$1.9  & 7.0 & $\pm$3.6 & 11.5  & $\pm$10.5 & 17.8 &
$\pm$0.4 & \colorbox{mine}{21.7} & $\pm$0.1 \\

\midrule
\multirow{3}{*}{\rotatebox[origin=c]{90}{Medium}} 

& HalfCheetah & 73.1 & $\pm$2.4  & 60.6 & $\pm$2.4 & 54.2 & $\pm$1.5 & \colorbox{mine}{77.6} &
$\pm$1.5 & 74.3 & $\pm$0.2 & 61.6 & $\pm$1.2 \\

& Hopper & 38.3 & $\pm$34.9  & 81.3 & $\pm$15.7  & 97.2 & $\pm$2.2  & 92.8 & $\pm$6.0 &
102.6 & $\pm$0.1 & \colorbox{mine}{104.2} & $\pm$0.6\\

& Walker2D & 41.2 & $\pm$30.8  & 85.3 & $\pm$1.3  & 81.9 & $\pm$2.8  & 85.0 & $\pm$15.0 &
\colorbox{mine}{95.5} & $\pm$0.4 & 87.9 & $\pm$1.1 \\

\midrule
\multirow{3}{*}{\rotatebox[origin=c]{90}{\shortstack{Medium\\Replay}}} 

& HalfCheetah & \colorbox{mine}{69.2} & $\pm$1.1  & 55.7 & $\pm$0.9 & 55.1 & $\pm$1.0 & 68.9 &
$\pm$2.3 & 66.4 & $\pm$0.3 & 58.0 & $\pm$0.6 \\

& Hopper & 32.7 & $\pm$9.4  & 69.0 & $\pm$27.0  & 89.5 & $\pm$2.8 & 96.6  & $\pm$7.0 &
\colorbox{mine}{104.3} & $\pm$0.4 & 101.5 & $\pm$3.1 \\

& Walker2D & 73.7 & $\pm$9.4  & 83.1 & $\pm$5.0 & 56.0 & $\pm$8.6 & 85.0 & $\pm$15.0 &
\colorbox{mine}{92.7} & $\pm$0.9 & 79.3 & $\pm$1.2 \\

\midrule
\multirow{3}{*}{\rotatebox[origin=c]{90}{\shortstack{Medium\\Expert}}} 

& HalfCheetah & 70.3 & $\pm$21.9  & 95.0 & $\pm$1.7 & 90.0 & $\pm$5.6 & 93.7 & $\pm$10.5 &
\colorbox{mine}{105.4} & $\pm$1.6 & 100.6 & $\pm$2.6 \\

& Hopper & 60.6 & $\pm$32.5  & 95.0 & $\pm$1.7 & \colorbox{mine}{111.1} & $\pm$2.9
& 83.3 & $\pm$9.1 & \colorbox{mine}{111.6} & $\pm$0.2 & 96.9 & $\pm$6.3 \\

& Walker2D & 77.4 & $\pm$27.9  & 107.7 & $\pm$0.8  & 103.3 & $\pm$5.6 & 68.3 & $\pm$20.6 &
\colorbox{mine}{117.2} & $\pm$0.5 & 108.4 & $\pm$0.7 \\

\midrule
\multicolumn{1}{l}{} & \textbf{Average} & \multicolumn{2}{c}{49.4} & \multicolumn{2}{c}{66.7} &
\multicolumn{2}{c}{66.8} & \multicolumn{2}{c}{68.7} &\multicolumn{2}{c}{\colorbox{mine}{79.3}}
&\multicolumn{2}{c}{72.4} \\

% \multicolumn{1}{l}{} & \textbf{Median} & \multicolumn{2}{c}{50.9} & \multicolumn{2}{c}{76.8} &
% \multicolumn{2}{c}{69.0} & \multicolumn{2}{c}{80.4} &\multicolumn{2}{c}{94.1}
% &\multicolumn{2}{c}{81.9} \\

% \multicolumn{1}{l}{} & \textbf{IQM} & \multicolumn{2}{c}{52.6} & \multicolumn{2}{c}{73.2} &
% \multicolumn{2}{c}{71.1} & \multicolumn{2}{c}{78.0} &\multicolumn{2}{c}{89.3}
% &\multicolumn{2}{c}{79.3} \\
\bottomrule

\end{tabular}
\end{table}

